Decodable Is Not Grounded: A Vision-Ablation Arbiter for VLM Spatial Reasoning

The standard way to read latent knowledge out of a model, a linear probe confirmed by a steering recovery, can systematically overstate what a vision-language model (VLM) actually grounds in the image. We show this on spatial reasoning, where the error is invisible to both probing and steering yet exposed by a one-line causal control: replacing the image with a gray blank. Probes decode the within-axis answer at 73--97% across axes, and a training-free projection lifts a near-chance axis from 59% to 79%, exactly the signature of unlocking latent knowledge. The blank-image arbiter refutes it, revealing three grounding regimes that probing conflates: an axis can be grounded (vision-dependent, correct), a prior (vision-independent, with its decode and its apparent recovery a directional default rather than perception), or, surprisingly, inverted: decodable, causally controllable, but deployed with the wrong sign, so the model scores below chance and the error requires looking. The taxonomy holds across the studied VLMs: in fourteen models spanning six language-model families and 2B--27B, horizontal is grounded, vertical is a prior, and depth is inverted, with the inversion emerging at scale within families. The decode-versus-deploy inversion replicates on seven of eight models across five families, and the minimal edit that re-deploys it varies with geometry: a training-free rotation matches a trained edit on the cleanest model, while distributed inversions need a trained low-rank edit, tracing a per-model correction-complexity spectrum. The cheap, self-calibrating arbiter cleanly separates grounded perception, inverted perception, and prior substitution; we argue it should be a default control for latent-knowledge and steering claims in VLMs.

==> figures/fig_method.tex <==
% =============================================================================
% Figure: correction-complexity spectrum -- training-free-best vs trained depth lift.
% Data: EXPERIMENT_LOG T25 (Run 17h). depth-acc lift over baseline, n~150.
% =============================================================================
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    width=0.74\linewidth, height=3.7cm,
    ybar=2pt, bar width=9pt,
    enlarge x limits=0.20,
    ymin=-8, ymax=65,
    ytick={0,10,20,30,40,50,60},
    ymajorgrids, grid style={gray!18},
    ylabel={\small depth-correction lift},
    symbolic x coords={Qwen3-VL-8B, Qwen2.5-VL-7B, Pixtral-12B, Qwen2.5-VL-3B},
    xtick=data, xticklabel style={font=\scriptsize, rotate=15, anchor=east},
    tick label style={font=\footnotesize},
    legend style={at={(0.5,1.04)}, anchor=south, legend columns=2,
                  font=\footnotesize, draw=neutralGray!50,
                  /tikz/every even column/.append style={column sep=0.4cm}},
    legend cell align=left,
    legend image code/.code={
      \draw[#1, draw=none] (0cm,-0.08cm) rectangle (0.35cm,0.13cm);
    },
    nodes near coords, nodes near coords style={font=\tiny, /pgf/number format/.cd, fixed, precision=1, print sign},
]
\addplot[draw=groundedTeal, fill=groundedTeal!28!white,
         error bars/.cd, y dir=both, y explicit, error bar style={neutralGray!80!black, line width=0.6pt}]
    coordinates {(Qwen3-VL-8B,55.7) +-(0,8) (Qwen2.5-VL-7B,15.5) (Pixtral-12B,2.4) (Qwen2.5-VL-3B,8.8)};
\addlegendentry{training-free best (rotation)}
\addplot[draw=accentBlue, fill=accentBlue!25!white,
         error bars/.cd, y dir=both, y explicit, error bar style={neutralGray!80!black, line width=0.6pt}]
    coordinates {(Qwen3-VL-8B,57.1) +-(0,2) (Qwen2.5-VL-7B,42.9) (Pixtral-12B,32.5) (Qwen2.5-VL-3B,-2.6)};
\addlegendentry{trained (LoRA)}
\draw[neutralGray!70, densely dotted] (axis cs:Qwen3-VL-8B,0) -- (axis cs:Qwen2.5-VL-3B,0);
\end{axis}
\end{tikzpicture}
\caption{\textbf{A correction-complexity spectrum: the minimal fix that re-deploys depth diagnoses the
inversion geometry.} Depth-accuracy lift over baseline (ViewSpatial depth, $n{\approx}150$). For
Qwen3-VL-8B the inversion is a clean low-dimensional rotation, so a \emph{training-free}
norm-preserving rotation ($+56$) matches a trained LoRA ($+57$). For the distributed inversion in
Qwen2.5-VL-7B and the ``decodable-but-not-installable'' inversion in Pixtral-12B, training-free edits
are weak and a trained low-rank edit is required ($+43$, $+33$). Qwen2.5-VL-3B is not inverted
(\S\ref{sec:crossmodel}), so nothing helps and training even hurts---the spectrum correctly flags it.
Which correction succeeds is thus a read-out of the inversion's geometry per model. Error bars on
Qwen3-VL-8B are $\pm1$ s.d.\ over three seeds (rotation $49\pm8$, trained $55\pm2$): the
training-free$=$trained tie is not a single-seed artifact. Values shown as percentages.}
\label{fig:method}
\end{figure}


==> figures/fig_teaser.tex <==
% =============================================================================
% Figure 1 (teaser): three grounding regimes -- real vs gray-blank image.
% Data: EXPERIMENT_LOG T19 (Run 11), Qwen2.5-VL-7B, ViewSpatial Cam-Rel.Dir.
% =============================================================================
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    width=0.92\linewidth, height=5.0cm,
    ybar=2pt, bar width=11pt,
    enlarge x limits=0.22,
    ymin=0.20, ymax=0.92,
    ytick={0.3,0.4,0.5,0.6,0.7,0.8,0.9},
    ymajorgrids, grid style={gray!18},
    ylabel={\small binary axis accuracy},
    symbolic x coords={Horizontal, Vertical, Depth},
    xtick=data,
    xticklabel style={font=\small},
    tick label style={font=\footnotesize},
    legend style={at={(0.5,1.04)}, anchor=south, legend columns=2,
                  font=\footnotesize, draw=neutralGray!50},
    nodes near coords, nodes near coords style={font=\tiny\bfseries},
    every node near coord/.append style={/pgf/number format/fixed,
                  /pgf/number format/precision=3},
]
\addplot[draw=groundedTeal, fill=groundedTeal!28!white] coordinates
    {(Horizontal,0.824) (Vertical,0.585) (Depth,0.314)};
\addplot[draw=neutralGray!90!black, fill=neutralGray!28!white] coordinates
    {(Horizontal,0.494) (Vertical,0.596) (Depth,0.451)};
\draw[densely dashed, neutralGray!90!black, thick]
    (axis cs:Horizontal,0.5) -- (axis cs:Depth,0.5);
\node[anchor=south, font=\tiny, neutralGray!90!black, fill=white, inner sep=0.6pt]
    at (axis cs:Depth,0.5) {chance $=0.5$};
\legend{real image, gray-blank image (vision ablated)}
\end{axis}
\end{tikzpicture}
\caption{\textbf{One causal control separates three grounding regimes.} Binary within-axis
accuracy of Qwen2.5-VL-7B on ViewSpatial Camera-Relative-Direction, with the real image vs.\
a same-size gray-blank image (vision ablated; question and options unchanged).
\textbf{Horizontal} collapses to chance when blinded $\Rightarrow$ \emph{grounded and correct}.
\textbf{Depth} sits below chance with the image but reverts to chance when blinded $\Rightarrow$
\emph{grounded but systematically inverted} (the error \emph{requires} the image).
\textbf{Vertical} is unchanged by removing the image $\Rightarrow$ the answer comes from a
\emph{linguistic prior, not vision} --- yet a linear probe decodes the vertical label at
$0.94$ accuracy (Fig.~\ref{fig:dissociation}). Decodability is not grounding.}
\label{fig:teaser}
\end{figure}


==> sections/08_limitations.tex <==
\subsection{Limitations}
\label{sec:limitations}

\paragraph{Scale-emergence is family-specific, not a clean law.} Depth-inversion emerges with LM scale
in three within-family ladders, but only two are monotone (InternVL3, Qwen2.5-VL); Gemma-3 emerges then
partially recovers at 27B (Fig.~\ref{fig:depth_scale}), and onset differs by family. We therefore claim
``emerges with scale within families,'' not a universal monotone trend, and the mechanism of the
recovery at the largest Gemma is unexplained. The capability-floor model (SmolVLM-2.2B, near chance on
all axes) bounds the ``horizontal universal'' claim to capable models and is read cautiously given its
prompt-format sensitivity.

\paragraph{The depth-type boundary is characterized behaviorally, not yet mechanistically.} We show the
depth inversion is specific to camera-egocentric front/back and absent on near-field front/behind and
metric closer-to-camera depth (\S\ref{sec:external}), a robust behavioral dissociation across models.
Why camera-egocentric framing specifically inverts---whether it is a viewpoint-transform failure, a
training-distribution effect, or a labeling convention---is not settled here and is the natural next
mechanistic target. Metric-depth ground truth (e.g.\ ScanNet) would further separate a true perceptual
inversion from a consistent internal convention.

\paragraph{The clean rotation tie is single-model; the population claim is broader.} The
\emph{inversion itself} now replicates on seven of eight models across five families
(\S\ref{sec:method}), so the decode$\neq$deploy phenomenon is not single-model. What remains
model-specific is the clean training-free$=$trained \emph{rotation} tie: it holds for Qwen3-VL-8B
(now over three seeds, $49\pm8$ vs.\ $55\pm2$, so not a single-seed artifact), while the rotation
works only partially or not at all on the other models, and distributed (Qwen2.5-VL-7B) and
not-installable (Pixtral-12B) inversions still require per-model trained edits that do not transfer
zero-shot. The headline is multi-seed; the per-model spectrum and card-C rung assignments elsewhere
are single-seed, and the card-C fingerprint is hyperparameter-sensitive at borderline models (stated
in \S\ref{sec:method}). Two auxiliary diagnostics are explicitly unreliable here and are not used as
evidence: a tiny-data overcomplete SAE (degenerate reconstruction) and a logit-lens trajectory that
does not support a ``computes-correctly-then-inverts'' reading---we claim only that depth never reaches
output-token space with the correct sign. The contribution is a diagnosis-to-correction arc in which
the correction's form is itself informative, not a turnkey fix.

\paragraph{Scope of the deep mechanism.} The full deep spine (path localization, vision-vs-LM
attribution, five-way arbiter) is run on the Qwen2.5-VL-7B anchor; we reproduce the core localization
and correction geometry on a second model and family (Qwen3-VL-8B, \S\ref{sec:method},
Table~\ref{tab:model2}), but the SigLIP-vision Gemma-3 family is absent from the correction battery
(an environment/toolchain constraint), so the correction-spectrum population is five families, not
six.

\paragraph{Scope.} The deep mechanism (probing, steering, projection, path localization) is on one
model; the taxonomy, the external task-type boundary, and the correction are shown on a model subset
rather than all fourteen. The depth splits are small per model and benchmark, so depth numbers are best
read as directional.


==> sections/09_conclusion.tex <==
\subsection{Conclusion}
\label{sec:conclusion}

We followed the standard latent-knowledge recipe on a VLM spatial axis: a probe decoded vertical
direction at $0.94$ while the model behaved at chance, and a training-free projection ``recovered'' it
to $0.79$ with the horizontal control intact. A one-line causal control---blanking the image, robust
across five ablations including an in-distribution mismatched image---showed the recovery to be
amplification of a non-visual ``default-to-above'' prior, and resolved the apparent dissociation into
three grounding regimes: horizontal (grounded and correct), depth (grounded and inverted), and vertical
(not grounded). Across fourteen models and six LM families the taxonomy and the finding that
decodability overstates grounded knowledge both hold, with depth inversion emerging with LM scale within
families. On external benchmarks the inversion sharpens into a task-type boundary---camera-egocentric
front/back inverts while near-field and metric depth are grounded---and the minimal correction that
re-deploys the inverted axis diagnoses its geometry: a training-free rotation suffices where the
inversion is a clean flip (matching a trained edit), while distributed inversions need a trained
low-rank edit. The lesson
is that linear decodability and steering pushability both overstate grounded spatial knowledge because
they are blind to whether behavior depends on the image, and that a cheap, self-calibrating
vision-ablation arbiter cleanly separates grounded perception, inverted perception, and prior
substitution. We recommend it as a default control for latent-knowledge and activation-steering claims
in VLMs. The open problems are now sharper: the mechanism of the camera-egocentric depth inversion and
its partial recovery at the largest scales, and whether a single trained correction can be made to
transfer across models.

